The Homogenization Problem in LLMs: Towards Meaningful Diversity in AI Safety

Generative AI models reproduce the human biases in their training data and further amplify them through mechanisms such as mode collapse. The loss of diversity produces homogenization, which not only harms the minoritized but impoverishes everyone. We argue homogenization should be a central concern in AI safety. To meaningfully characterize homogenization in Large Language Models (LLMs), we introduce a framework that allows stakeholders to encode their context and value system. We illustrate our approach with an experiment that surfaces gender bias in an LLM (Claude 3.5 Haiku) on an open-ended story prompt. Building from queer theory, we formalize homogenization in terms of normativity. Borrowing language from feminist theory, we introduce the concept of xeno-reproduction as a class of tasks for mitigating homogenization by promoting diversity. Our work opens a collaborative line of research that seeks to understand and advance diversity in AI.

==> figures/dynamics-trace.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\columnwidth]{images/dynamics-magnitude.png}
    \Description{Line chart tracing the L2 magnitude of pull, drift, and potential along a single generated trajectory token by token.}
    \caption{The potential drops to zero while drift converges to initial value of potential.}
    \label{fig:dynamics-trace}
\end{figure}

